Beyond symmetrization: effective adjacency matrices and renormalization for (un)singed directed graphs

To address the peculiarities of directed and/or signed graphs, new Laplacian operators have emerged. For instance, in the case of directionality, we encounter the magnetic operator, dilation (which is underexplored), operators based on random walks, and so forth. The definition of these new operators leads to the need for new studies and concepts, and consequently, the development of new computational tools. But is this really necessary? In this work, we define the concept of effective adjacency matrices that arise from the definition of deformed Laplacian operators such as magnetic, dilation, and signal. These effective matrices allow mapping generic graphs to a family of unsigned, undirected graphs, enabling the application of the well-explored toolkit of measures, machine learning methods, and renormalization groups of undirected graphs. To explore the interplay between deformed operators and effective matrices, we show how the Hodge-Helmholtz decomposition can assist us in navigating this complexity.

==> applications.tex <==
\section{Results}


==> methods/reno.tex <==
\subsection{Renormalization procedures}


Going back to the three main questions motivating our approach, we observe that questions \ref{question1} and \ref{question2} are not immediately related to question
\ref{question3}.  

However, it is possible to use a coarse-graining procedure in the adopted hidden spaces so as to derive a relationship among spectrum, structure and dynamics in complex networks using hidden metric spaces as a intermediary concept,  as explained in the following. 

Let us consider the problem of studying how a measurement $\mathcal{M}$ on a graph $G^{(0)}=(V, E, w)$ is related to the adopted hidden spaces, and consequently with the respective dynamics whit generates the embedding into this space.  First, we map $G$ into a metric space $S$, so that each vertex $u\in V$ becomes associated with a point $\mathbf r^{(0)}_u \in S$.  Therefore, the embedding yielding a set of points $\{r^{(0)}_u\}$, as shown in\figref{figCvEVO3FLUX}(e). By construction, it follows that the proximity between vertices in this space is related to the similarity of some  property (e.g.~frustration or dynamics in phase space).
Now, we can define a coarse-graining procedure resembling those used in statistical mechanics~\cite{kadanoff1966scaling,NaturePhysicsRenormalizaton2018}. 

After make the measurement of $\mathcal{M}$ in $G^{(0)}$ , $\mathcal M^{(0)}$, and embedding the graph in the hidden  space,  $\{r^{(0)}_u\}$ we  group vertices  into super-vertices such that the sum of the distances (some metric  must be used, here we are using the Euclidean metric)  between its constituent elements be as small as possible. Each super-vertex represents a vertex of a new graph  $G^{(1)}= (\frac{|V|}{2}, E^{(1)}, w^{(1)} )$, as illustrated in Figure\figref{figCvEVO3FLUX}(c); where $E^{(1)}$ and $w^{(1)}$ 
can be defined so as to preserve some specific property of the original network.  Now, we calculate $\mathcal M$ in $G^{(1)}$, $\mathcal{M}^{(1)}$, and map $G^{(1)}$ into $S$, defining a new set of positions associated to the vertices $\{\mathbf r^{(1)}_u\}$. This renormalization procedure can be repeated for a given number of stages, as shown in\figref{figCvEVO3FLUX}(a).  At the end,  this coarse grained procedure provides the flow
\begin{align}
	\begin{rcases}
		G^{(0)} \\
		\mathcal{M}^{(0)} \\
		\{r^{(0)}_u\}
	\end{rcases}
	\mapsto
	\begin{rcases}
		G^{(1)} \\
		\mathcal{M}^{(1)} \\
		\{r^{(1)}_u\}
	\end{rcases}
	\mapsto
	\dots
	\mapsto
	\begin{rcases}
		G^{(N)} \\
		\mathcal{M}^{(N)} \\
		\{r^{(N)}_u\}
	\end{rcases},
\end{align}

As a proof of concept of using aforementioned coarse-graining procedure we choose to better understand the relationship between the specific heat measurement and the hidden spaces of modular directed networks.  In order to do so, we created a  modular directed network  with $N_f=3$, $p_c=50\%$, $p_d=70\%$ and $|V|=300$. The mapping  $c_\lambda$  of this network is shown in\figref{figCvEVO3FLUX}(f). The petal structures obtained for the specific heat are a consequence of modular structures (communities) in the network, as discussed in the Supplementary Material \ref{secSupMatStructureAndCv}. Therefore, we  expect that petal structures  must be preserved during coarse-graining procedure if this structures is correlated with  the positions in the hidden metric space. In other words, if the behavior of $c_\lambda$  is correlated with the macrostrutures in the hidden spaces, we expect then lows scales to vanish in this space, and, if connections among super-vertices are preserved, the behavior of $c_\lambda$ also remains unchanged.  


